Closing the Reality Gap: Zero-Shot Sim-to-Real Deployment for Dexterous Force-Based Grasping and Manipulation

Human-like dexterous hands with multiple fingers offer human-level manipulation capabilities, but training control policies that can directly deploy on real hardware remains difficult due to contact-rich physics and imperfect actuation. We close this gap with a practical sim-to-real reinforcement learning (RL) framework that utilizes dense tactile feedback combined with joint torque sensing to explicitly regulate physical interactions. To enable effective sim-to-real transfer, we introduce (i) a computationally fast tactile simulation that computes distances between dense virtual tactile units and the object via parallel forward kinematics, providing high-rate, high-resolution touch signals needed by RL; (ii) a current-to-torque calibration that eliminates the need for torque sensors on dexterous hands by mapping motor current to joint torque; and (iii) actuator dynamics modeling to bridge the actuation gaps with randomization of non-ideal effects such as backlash, torque-speed saturation. Using an asymmetric actor-critic PPO pipeline trained entirely in simulation, our policies deploy directly to a five-finger hand. The resulting policies demonstrated two essential skills: (1) command-based, controllable grasp force tracking, and (2) reorientation of objects in the hand, both of which were robustly executed without fine-tuning on the robot. By combining tactile and torque in the observation space with effective sensing/actuation modeling, our system provides a practical solution to achieve reliable dexterous manipulation. To our knowledge, this is the first demonstration of controllable grasping on a multi-finger dexterous hand trained entirely in simulation and transferred zero-shot on real hardware.

==> Other/paper_clone.tex <==
\title{Closing the Reality Gap: Zero-Shot Sim-to-Real Deployment for Dexterous Force-Based Grasping and Manipulation}


\abstract{
Human-like dexterous hands with multiple fingers offer human-level manipulation capabilities but remain difficult to train the control policies that can deploy on real hardware due to contact-rich physics and imperfect actuation. We present a sim-to-real reinforcement learning that leverages dense tactile feedback combined with joint torque sensing to explicitly regulate physical interactions. To enable effective sim-to-real transfer, we introduce (i) a computationally fast tactile simulation that computes distances between dense virtual tactile units and the object via parallel forward kinematics, providing high-rate, high-resolution touch signals needed by RL; (ii) a current-to-torque calibration that eliminates the need for torque sensors on dexterous hands by mapping motor current to joint torque; and (iii) actuator dynamics modeling with randomization to account for non-ideal torque–speed effects and bridge the actuation gaps. Using an asymmetric actor–critic PPO pipeline, we train policies entirely in simulation and deploy them directly to a five-finger hand. The resulting policies demonstrated two essential human-hand skills: (1) command-based controllable grasp force tracking and (2) reorientation of objects in the hand, both of which were robustly executed without fine-tuning on the robot. By combining tactile and torque in the observation space with scalable sensing/actuation modeling, our system provides a practical solution to achieve reliable dexterous manipulation. To our knowledge, this is the first demonstration of controllable grasping on a multi-finger dexterous hand trained entirely in simulation and transferred zero-shot on real hardware.
}



\section{Introduction}
\label{sec:intro}
Multi-finger dexterous hands offer human-like manipulation potential, yet their high degrees of freedom (DoFs) and complex contact dynamics pose substantial control challenges. As a result, most robotic applications still rely on simpler parallel-jaw grippers, and achieving robust in-hand manipulation remains a research challenge in robotics.

%This research particularly investigates the use of \emph{full-state} feedback, including tactile sensing and joint torques, for learning manipulation policies that can explicitly sense and regulate contact. In contrast to vision- or kinematics-only approaches, we feed the policy with high-resolution tactile feedback \emph{and} joint-level torques, which represent the interaction forces exerted by multi-fingers. With use of “touch-and-torque” observation, we formulate the reinforcement learning (RL) objectives to achieve effective learning of two essential manual skills—(i) \emph{controllable grasping} (tracking commanded grip forces), and (ii) \emph{in-hand reorientation}.

This work focuses on using the \textit{full-state} feedback, including tactile sensing and joint torques, to learn manipulation policies capable of explicitly sensing and regulating contact. Unlike vision- or kinematics-only methods, our policy uses high-resolution tactile sensing and joint-level torques, capturing fine-grained interaction forces during multi-finger manipulation. This ``touch \& torque'' observation supports reinforcement learning (RL) objectives for two fundamental manual skills: (i) force-controllable grasping (tracking commanded grip forces), and (ii) in-hand reorientation.

Deep reinforcement learning (RL) has begun to unlock dexterous in-hand skills. A landmark result trained a five-finger hand to rotate objects purely in simulation and transferred it to a real robot via large-scale domain randomization~\cite{andrychowicz2018learning}, with subsequent work culminating in automatic domain randomization for a Rubik’s Cube~\cite{akkaya2019rubik} and establishing sim-to-real as a key tool~\cite{tobin2017dr}. 

%Deep reinforcement learning (RL) has emerged as a promising approach for dexterous in-hand manipulation. Related work demonstrated that policies trained in simulation with large-scale domain randomization could be transferred to a real five-finger hand to rotate objects~\cite{andrychowicz2018learning}. Subsequently, automatic domain randomization for a Rubik’s Cube~\cite{akkaya2019rubik} has shown that sim-to-real can be a key tool~\cite{tobin2017dr}. Recent efforts improved simulation fidelity and robustness to train with extensive randomization which yields robust cube reorientation on an Allegro Hand~\cite{handa2023dextreme}. Beyond vision-only policies, recent results integrating tactile sensing has significantly enhanced dexterity, e.g., combining visuotactile and point-cloud inputs~\cite{yuan2023robotsynesthesia} and achieving in-hand rotation using only dense binary touch signals~\cite{yin2023rotating}. Progress also extends to dexterous grasping~\cite{zhang2025robustdexgrasp} and contact-rich humanoid skills~\cite{lin2025humanoid}. Together, these results suggest that with the right sensing and modeling, \emph{sim-to-real RL} can learn manipulation policies readily deployable on real hardware.


Deep reinforcement learning (DRL) has emerged as a promising approach for dexterous in-hand manipulation. Work by ~\cite{andrychowicz2018learning} demonstrated that large-scale domain randomization could transfer simulated object rotation policies to a real five-finger hand. Subsequent advances, such as automatic domain randomization for solving a Rubik’s Cube~\cite{akkaya2019rubik}, and showed sim-to-real as a key tool~\cite{tobin2017dr}. Recent efforts improved simulation fidelity and robustness to train with extensive randomization which yields robust cube reorientation on an Allegro Hand~\cite{handa2023dextreme}. Beyond vision-only policies, integrating tactile sensing has significantly improved dexterity, e.g., fusing visuotactile and point-cloud inputs~\cite{yuan2023robotsynesthesia}, and and achieving in-hand rotation using only dense binary touch signals~\cite{yin2023rotating}. Progress also extends to dexterous grasping~\cite{zhang2025robustdexgrasp}, dexterous in-hand manipulation of thin objects with binary tactile sensing~\cite{hu2025dexterous}, and contact-rich humanoid skills~\cite{lin2025humanoid}. All these results suggest that with the right sensing and modeling, \emph{sim-to-real RL} can learn policies readily deployable on real hardware.


% Recent works report encouraging progress by improving simulation fidelity and policy robustness. ~\cite{handa2023dextreme} demonstrates robust cube reorientation on an Allegro Hand via simulation and extensive randomization. Beyond vision-only policies, integrating tactile sensing can further enhance sim-to-real dexterity: ~\cite{yuan2023robotsynesthesia} fuses visuotactile inputs with a point-cloud tactile representation to perform in-hand rotations, while ~\cite{yin2023rotating} achieves in-hand rotation using only dense binary touch sensing and direct zero-shot deployment. Progress also extends to dexterous grasping: ~\cite{zhang2025robustdexgrasp} reports strong zero-shot grasp success on 500+ real objects, and recent work on humanoids advances sim-to-real RL for contact-rich, vision-based dexterity~\cite{lin2025humanoid}. Together, these results suggest that with the right techniques—better sensing, realistic actuation models, and targeted randomization—\emph{sim-to-real RL} can unlock agile manipulation on real hardware.


However, there are two practical hurdles for full-state policies that use tactile sensing and joint torques: (i) \textbf{Simulation of dense tactile contacts}. Simulating high-resolution tactile/contact is computationally too slow for massive RL exploration, resulting in a brittle policy due to insufficient exploration of contact dynamics. (ii) \textbf{Discrepancies of actuator dynamics and modeling}. Most dexterous hands have semi-direct-drive actuation with no direct joint torque sensors and thus rely on the motor current to estimate the joint torques, where inaccuracies and uncertainties in the actuator dynamics can hurdle the sim-to-real transfer. In short, major gaps in the \textit{modeling and simulation of surface contacts of tactile sensors and the mechatronic properties of actuators} prevent full-state policies from being fully exploited for policy learning. 

% As high-DoF dexterous robotic hands become more commercially available, we are motivated to investigate the sim-to-real \textit{recipe} for learning \textit{full-state policies} for dexterous hands (including tactile sensing and joint torque), to address these bottlenecks by effective modeling of contacts and actuation. Our method trains a policy on a five-finger hand entirely in simulation and deploys it directly to the real world. Specifically, the contribution of sim-to-real \textit{recipe} includes:

As high-DoF dexterous hands become more available, we are motivated to develop a reliable sim-to-real \textit{recipe} for learning full-state policies (including tactile sensing and joint torques) that address key sim-to-real gaps through effective modeling of tactile sensors and actuators. Our method trains a policy in simulation and deploys it directly to a real five-finger hand. The contributions of this \textit{recipe} include:
\begin{itemize}
[leftmargin=*]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
\item \textbf{Full-state policies.} We formulate the policy observations that jointly intake dense tactile sensing and joint torques, enabling explicit feedback that can infer contact states and contact forces.
\item \textbf{Fast, high-resolution tactile simulation.} We approximate tactile contacts by computing distances between a dense array of \emph{virtual tactile units} and the object via parallel forward kinematics, offering more accurate, high-rate tactile feedback suitable for massive RL training.
\item \textbf{Data-driven actuator modeling.} We bridge the sim-to-real actuation gap by calibrated current-to-torque mapping and randomization to account for uncertain motor dynamics (e.g., torque-velocity curves), requiring no direct torque sensors and reducing sim-to-real torque discrepancies on real hardware.
% \item \textbf{Motor dynamics modeling and randomization.} We capture non-idealities (e.g., torque–speed limits) and randomize key parameters during training to bridge actuation gaps.
\item \textbf{Contact-rich sim-to-real RL policy training.} We trained and deployed two contact-rich skills: (1) \emph{controllable grasping} that tracks commanded grip forces and (2) \emph{in-hand object reorientation} -- full-state policies directly deployed for force-modulated grasps and reorientations on the real robot.
\end{itemize}

%In summary, we contributed an easy-to-replicate \textit{recipe} for training full-state RL policies on a representative dexterous hand (12-DoF) widely available for robotics research. By combining tactile/torque-aware observations with approximate tactile simulation, actuator calibration, and modeling of motor dynamics, our \textit{recipe} achieves zero-shot transfer of \emph{force-controllable} grasping and in-hand reorientation with policies trained entirely in simulation. To the best of our knowledge, this is the first demonstration of \emph{controllable grasping} with controllable grip-force tracking, force-adaptive grasping, and robust in-hand manipulation on a dexterous multi-finger hand.

In summary, this serves as an easy-to-replicate \textit{handbook} for training full-state RL policies on a representative dexterous hand (12-DoF) widely available recently for robotics research. Our approach integrates tactile and motor-current sensing with computationally efficient simulation and robust actuator modeling, enabling zero-shot sim-to-real transfer of force-controllable grasping and in-hand manipulation. To the best of our knowledge, this is the first demonstration of \emph{controllable grasping} with grip-force tracking, force-adaptive grasping, and robust in-hand manipulation on a dexterous multi-finger hand.

%To the best of our knowledge, this is the first demonstration of direct sim-to-real transfer of force-sensitive dexterous manipulation on a multi-fingered hand.


\section{Related Work}
\label{sec:related_work}
We review research work closely related to our focused techniques in our sim2real pipeline for dextrous hands: (i) simulation of tactile sensors, (ii) modeling of motor dynamics, and (iii) current-to-torque mapping and estimation without direct joint torque sensors.
% , and (iv) dexterous manipulation tasks and sim-to-real RL on other robot morphologies.

\subsection{Tactile Simulation}
High-fidelity, fast tactile simulation is a long-standing obstacle for learning contact-rich skills. For visuotactile sensors, recent systems libraries have pushed both realism and throughput. Akinola \emph{et al.} builds a library within Isaac Gym that synthesizes visuotactile images and contact-force distributions, and couples them with a policy-learning toolkit aimed at sim2real transfer~\cite{akinola2025tacsl}. In parallel, Nguyen \emph{et al.} integrate a soft-body FEM simulator with an optical visuotactile rendering pipeline inside Isaac Sim to capture elastomer deformation for GelSight-like skins~\cite{nguyen2024tacex}. Zhang \emph{et al.} focus on modeling multi-mode tactile imprints induced by different surface coatings/patterns and report high realism while remaining efficient enough for learning loops~\cite{zhang2025tacflex}. Beyond single-hand settings, works begin to exploit visuo–tactile simulation for complex, often bimanual, fine assembly: e.g., general sim2real protocols for marker-based visuotactile sensors~\cite{chen2024gpvt}, bimanual visuotactile assembly via simulation fine-tuning~\cite{huang2025vtrefine}.

On the policy side, tactile-only or visuo–tactile in-hand reorientation has seen rapid progress. Yin \emph{et al.}learns touch-only in-hand rotation on low-cost binary sensors, emphasizing robustness to sensing imperfections~\cite{yin2023rotating}. Yuan \emph{et al.} propose a point-cloud tactile representation to fuse vision and touch for in-hand rotation~\cite{yuan2024robotsynesthesia}. Purely tactile in-hand manipulation with a torque-controlled hand was shown in~\cite{sievers2022tactile}, while works also demonstrate DRL-based tactile control for slender cylindrical objects~\cite{hu2025slender}. For broader dexterous/bimanual touch, Lin \emph{et al.} studies bimanual tactile manipulation with sim-to-real deep RL~\cite{lin2023bitouch}. Collectively, these efforts motivate fast, high-fidelity tactile simulation and policy training; our distance-field–based tactile simulation targets this efficiency–fidelity trade-off specifically for RL.

% Robotic tactile sensing has seen significant progress in simulation frameworks and learning approaches. Recent libraries like TacSL (taxel) accelerate visuotactile sensor simulation by over 200× in NVIDIA Isaac Sim, providing multiple sensor models and contact-rich environments to facilitate policy learning with touch~\cite{akinola2025tacsl}. Similarly, TacEx integrates a soft-body physics engine (GIPC) with vision-based tactile rendering to simulate GelSight sensors in Isaac Sim, enabling stable high-dimensional tactile observations (gel deformations, RGB images) for training RL agents~\cite{nguyen2024tacex}. Another notable work is TacFlex, which introduces a multimodal tactile imprint simulation for optical tactile sensors with patterned coatings, improving realism of contact feedback (e.g. shear and normal force visualization) in simulation~\cite{zhang2025tacflex}. These advances in simulating visuotactile sensors have laid the groundwork for learning complex manipulation tasks with tactile feedback.

% Leveraging such simulations, researchers have tackled both single-hand and bimanual tactile manipulation. For example, Yin et al. propose TouchDexterity, which learns in-hand object rotation using only touch sensing – an Allegro hand outfitted with binary force sensors on the fingers and palm~\cite{yin2023rotating}. ~\cite{sievers2022tactile} demonstrate a purely tactile in-hand manipulation task on the torque-controlled DLR-Hand II, where an RL policy learned to continuously reorient a cube with the palm facing down (requiring constant force closure). Notably, this was achieved without any cameras or object pose input, relying only on joint proprioception and torque cues. Hu et al. focus on manipulating slender cylindrical objects (a thin stick) using high-resolution fingertip tactile arrays~\cite{hu2025slender}. 

\subsection{Motor Modeling}
% Accurate actuator modeling in simulation is central to closing dynamics gaps. In legged and humanoid systems, previous works demonstrate that careful actuator modeling, together with DR and SysID, enables agile skills to transfer: ANYmal’s agile locomotion~\cite{hwangbo2019agile}, soccer skills on low-cost humanoids~\cite{haarnoja2024soccer}, humanoid whole-body motion alignment via residual action modeling (\textsc{ASAP})~\cite{he2025asap}, and athletic loco-manipulation with actuator-gap learning (\textsc{UAN})~\cite{fey2025uan}. Reviews on model identification emphasize physically consistent parameterization and drive modeling as prerequisites for robust control and sim2real~\cite{lee2024robotid,gaz2019panda}.  

For dexterous hands and manipulation, recent systems explicitly incorporate motor/drive limits or task-informed SysID. Huang \emph{et al.} employ privileged learning, SysID, and DR to transfer functional grasps across diverse hands~\cite{huang2024fungrasp}. Tactile in-hand works with torque-controlled hands to build policies on top of explicit joint torque models~\cite{sievers2022tactile,hu2025slender}. In non-prehensile manipulation, early sim-to-real studies showed the importance of accurate actuation/friction models plus ensemble dynamics to combat identification error~\cite{lowrey2018nonprehensile}.  

In our setting, we explicitly model the motor’s \emph{torque–speed} envelope~\cite{shin2023actuatorconstrainedreinforcementlearninghighspeed}, then \emph{randomize} these parameters (stall torque, speed constants, friction/ripple surrogates) to cover manufacturing tolerances and temperature/load variation. This follows the spirit of recent agile-mobility works where actuator models are aligned via residual learning or unsupervised actuator nets~\cite{he2025asap,fey2025uan}, but adapts them to the brushed-DC, gear-driven fingers typical of dexterous hands.

\subsection{Current-to-Torque Alignment}
Most dexterous hands available nowadays typically have their SDKs to send over measurements of {motor current} but lack direct torque sensors at the joint level of the robot. When torque feedback (or torque-conditioned policy inputs) is desired, estimating a reliable \emph{current$\to$torque} mapping becomes critical. In industrial manipulator literature, motor-current–based wrench estimation has a long history: Kalman filtering and momentum-observer formulations are used to estimate Cartesian forces and torques from joint currents and states~\cite{wahrburg2017tase,han2022sensorless}. 
Gold \emph{et al.} consider torsional deflection plus motor current to estimate joint torques~\cite{gold2019ifac}. 
From the calibration and control perspective, current-based impedance control explicitly fits actuator current-torque ratios and friction for current-controlled robots--eschewing force-torque sensors, bypassing the need for force-torque sensors~\cite{dewolde2024currentimpedance}. System identification methods that identify the models and parameters of the drive gains and dynamics to ensure that the modeled dynamics is physically consistent with the real measurements~\cite{gautier2014drivegains}.  


% Compared to these, we target \emph{brushed-DC} finger actuators in dexterous hands. We fit a current$\to$torque map under quasi-static conditions to capture effective torque constants and biases (including gear train losses), Empirically, this provides torque observables for policies and improves sim–real alignment without adding expensive joint-torque sensors.

In this work, we adapt and apply these principles to the small electric motors that are commonly in dexterous hands for the design of direct-drive or semi-direct-drive of the joints. We fit a ``current$\to$torque map'' under quasi-static conditions to capture effective torque constants and biases, accounting for the a minor loss of torque exertion due to the \textit{wear-and-tear} of the gear train. Empirically, this mapping provides sufficiently accurate torque estimates for the RL policies and improves sim-to-real alignment,without physically building and embedding expensive miniaturized joint-torque sensors in the robot joints.

% \subsection{Dexterous Manipulation Tasks and Sim2Real RL}
% Pioneering works established zero-shot sim-to-real for in-hand reorientation via large-scale DR~\cite{andrychowicz2018learning}, and later, agile in-hand manipulation on affordable hardware with Isaac Gym~\cite{handa2022dextreme}. Visuo–tactile in-hand pipelines~\cite{yuan2024robotsynesthesia,yin2023rotating} and robust dexterous grasping from single-view perception~\cite{zhang2025robustdexgrasp} broaden the perceptual front-end. Beyond hands, robust sim2real RL on quadrupeds and humanoids provides strong evidence that principled randomization plus actuator/dynamics alignment scales to high-agility settings~\cite{hwangbo2019agile,haarnoja2024soccer,he2025asap,fey2025uan}.  

% Our study complements this line by emphasizing three \emph{sim2real enablers} tailored to low-cost dexterous hands: (1) parallel tactile simulation for RL data efficiency, (2) sensorless current-to-torque calibration to unlock torque-aware policies, and (3) motor modeling with parameter randomization (torque–speed envelope) to reduce actuator mismatch. We demonstrate two representative skills—force-scaled grasping and in-hand reorientation—trained entirely in simulation and transferred directly to hardware.
\section{Methodology}
\label{sec:method}
This section first presents the problem formulation, i.e., controllable grasping and in-hand object reorientation. Then, we present the technical details of our full-state policy learning framework, including the design of the full-state observation and the recipe of sim-to-real transfer.

\subsection{Problem formulation}
This work addresses the \textbf{sim-to-real transfer} of dexterous manipulation policies for multi-fingered robotic hands, focusing on zero-shot deployment of simulation-trained policies onto real hardware. Despite progress in RL-based manipulation, transferring contact-rich, force-sensitive tasks—such as variable-force grasping and in-hand reorientation—remains challenging due to gaps in tactile simulation, actuator modeling, and contact physics.

Formally, given a dexterous hand with $N$ fingers equipped with tactile sensors and current-controlled motors (no torque sensors), we learn a policy $\pi:o_t\mapsto a_t$ that maps observations in simulation that performs successfully on the physical system without fine-tuning.


\subsubsection{Force-Adaptive Grasping}
The objective of this task is to achieve and maintain stable grasps on a diverse set of objects with geometrically complex and physically varied properties—including size, shape, mass distribution, and surface friction—while accurately exerting user-specified force levels. The policy must modulate grip forces in real time according to object characteristics and external disturbances to prevent slip or excessive deformation, thereby demonstrating robust and adaptive grasping under dynamic real-world conditions.

\subsubsection{In-Hand Object Rotation}
This task requires the precise and controlled rotation of a grasped object about a predefined spatial axis using continuous and compliant finger gaits. Successful rotation entails rich, multi-point frictional contacts and requires coordinated finger motions that induce controlled slip and rolling interactions between fingertips and the object surface. The policy must maintain stability during manipulation by adjusting contact forces and reposing fingers as needed to avoid dropping or losing control of the object, thereby achieving smooth and continuous rotational reorientation.

Experiments use a 12-DoF direct-drive dexterous hand (XHand)~\cite{robotera2024generic} and are conducted in the IsaacLab simulation environment~\cite{mittal2023orbit}.
% \subsectionIdentification of Sim-to-Real Gaps}
% Three major Sim-to-Real Gaps:
% 1. Visual gap from cameras, in simulation, ground truth is used. In real we obtain visual feedback via cameras, the estimation of object related feedback needs to be achieved via extrinsic photon-based measurement.
% 2. Mechanical properties and dynamics of actuators. such as mechanical backlash of joints, servo control and actuator dynamics of motor units. 
% 3. Discrepancies of object-hand contact properties during contact-rich interactions. Such as mechanical structure of the hand, rubber pads in palm and fingertips which are not explicitly modeled, as well as object stiffness, friction, restitution, and so on. 
% 4. Last but not least, the state observations seen in the real deployment which were not previously observed in simulated environment. 

\subsection{Identification of Sim-to-Real Gaps}
Our study identified 4 primary sim-to-real gaps:

\textit{(1) Perceptual Gap:} Simulations often provide perfect ground-truth state information, such as object pose, joint angles. However the real systems rely on these states from noisy sources, including errors from camera calibration, varying lighting conditions, occlusions, and the limitations of vision-based pose estimation, resulting in a unavoidable mismatch between the policy's ideal expected observations and the actual ones.

% Unmodeled joint-level discrepancies such as transmission backlash, nonlinear motor control, and response delays.
\textit{(2) Discrepancies in Actuator Dynamics:} Real actuators, such as the commonly used electric motors, have complex and non-ideal behaviors that are often simplified or omitted in the physics simulation. It ranges from significant mechanical discrepancies in the physical gear chain system, such as mechanical backlash in gear transmissions, to nonlinearities such as static (stiction) and dynamic friction, torque-speed curves (e.g., motor current saturation at higher velocities), motor response delays, and imprecise current-to-torque mapping. These unmodeled acutator dynamics cause the commanded actions in reality exert different forces and thus exhibits different motion patterns on the real robot.

% Inaccurate contact modeling due to simplified surface geometry, material properties (e.g., stiffness, friction), and restitution.
\textit{(3) Discrepancies in Contact Physics:} The contact dynamics in the simulation is primarily based on rigid bodies, which often have limited accuracy in surface geometry due to the use of simpflied meshes, and also miss out the material properties (e.g., stiffness, friction, restitution) which are more complex to numerically compute. Therefore, for ensuring reasonable computational cost,  to some extent, most available simulation engines nowadays trade off the complexity and fidelity of real physical interactions, including multi-contact modeling, deformation of soft and compliant materials, varying friction coefficients, rolling resistance, and the stiffness-damping properties of the building materials of the robot. All these result in policies that fail to effectively explore and exploit rich tactile feedback in simulation, which is essential for dexterous in-hand manipulation.


% Mismatch between training and real-world observations during deployment. 
\textit{(4) Unseen State Distribution Shift:} Given the above main sources of discrepancies, even with robust training with randomization of key physical properties, a policy may still encounter novel object properties such as materials, shapes, masses, frictions--scenarios and configurations that are not exactly the same or not seen during training. This Out-of-Distribution (OOD) problem leads to compounding errors as the policy operates in those states where its learned value functions and policies are no longer accurate, causing performance deterioration or even failures while deployed in the real system.


\subsection{Data collection and curation}
\subsubsection{Force-adaptive grasping} 
Traditional dexterous grasping methods imitate human scenarios: objects are placed on a table and the hand starts from a random pose to attempt grasping. This approach requires extensive exploration, is computationally expensive, and often leads to unnatural grasps that fail in real environments due to sim-to-real gaps. To address these issues, we introduce an inverted ``catch-the-object'' setup where the hand is fixed upside down and objects are dropped toward the palm as shown in Fig.~\ref{fig:grasp}. The policy learns to catch and stably grasp objects under randomized object properties, dynamics, and external perturbations. This setup simplifies learning through natural gravity assistance, reduces reward exploitation, and produces robust grasping behaviors using only real-world measurable observations, facilitating better sim-to-real transfer.



\subsubsection{In-Hand Object Rotation}
% For the object rotation task, we use a cube as the rotating object. Due to the limitations in the degrees of freedom of the dexterous hand, we constrain the agent to rotate the cube along a single axis. To enable continuous rotation, we define a target pose as a 90-degree rotation from the initial pose about the specified axis. In the simulation environment, each 90-degree rotation of the cube about this fixed axis is considered a successful step. Upon each success, the target pose is updated by applying another 90-degree rotation from the current target pose along the same axis.
For the in-hand object rotation task, a standardized cube is employed as the manipulation object. Owing to the limited degrees of freedom (DoF) of the adopted dexterous hand, the agent is constrained to rotate the cube solely around a single, predefined axis. To facilitate continuous and sustainable rotational manipulation, the target pose is defined as a 90-degree increment relative to the object’s current orientation about that axis. Within the simulation environment, each instance of a successful 90-degree rotation around the designated axis is recorded as a successful step. Following each achievement, the target pose is dynamically updated by applying an additional 90-degree rotation relative to the most recent target, thus maintaining persistent rotation about the same fixed axis.

\subsection{Policy learning in simulation}



\subsubsection{Force-adaptive grasping} 
The complete set of observations used during policy training is detailed in Table~\ref{tab:RewardGrasping}. In the real-world deployment setup, the object’s three-dimensional position is estimated through a vision-based pipeline: the Z-coordinate is computed from the distance between the palm center and the centroid of the segmented object mask, where the mask is inferred using the Segment Anything Model (SAM)~\cite{kirillov2023segment}. The X and Y coordinates are held fixed relative to the hand’s initial pose, simplifying the state estimation under the assumption of limited lateral motion during grasping. The object’s linear velocity is then numerically derived from the sequence of estimated Z-coordinates using a finite difference method. Additionally, a force command scalar in the range [0, 1] is provided as part of the observation, indicating the desired grasping intensity—enabling the policy to modulate grip force according to task requirements.
During the simulation training process, we designed a reward mechanism to guide the policy toward achieving stable and reliable grasping during inverted catching tasks.

Once the fingers are in contact with the object, we employ torque command rewards $R_{\text{torque}}$ to encourage the agent to apply specific joint torques. The target torque $\tau_{\text{target}}$ is a continuous value provided by the instruction of the environment, and the reward function has a special handling for the thumb compared to the other fingers.

The total reward for this component is the sum of the individual finger torque rewards, which is applicable only when the finger is in contact with the object.
\begin{equation}
R_{\text{torque}} = w_{\text{torque}} \cdot \sum_{i \in \text{fingers}} R_{\text{torque}, i} \cdot I_{\text{contact}, i},
\end{equation}where $w_{\text{torque}}$ is the weight of this reward, $I_{\text{contact}, i}$ is the indicator function, which is 1 if the finger $i$ is in contact with the object and 0 otherwise.


The reward for the thumb is binary, contingent on its torque $R_{\text{torque, thumb}}$ being within a valid range:
\begin{equation}
R_{\text{torque, thumb}} = I(0.01 \le \tau_{\text{thumb}} \le 1.1),
\end{equation}

Other four fingers' reward is a Gaussian function centered around the instructed target, multiplied by a validity mask.
\begin{equation}
R_{\text{torque}, i} = \exp\left(-\frac{(\tau_i - \tau_{\text{target}})^2}{2\sigma^2}\right) \cdot I(0.01 \le \tau_i \le 1.1) ,\quad
\end{equation}

For the contact force, similar to the joint torque reward, an appropriate contact force is encouraged.
\begin{equation}
R_{\text{force}} = w_{\text{force}} \cdot \sum_{i \in \text{fingers}} R_{\text{force}, i} \cdot I_{\text{contact}, i},
\end{equation}
\begin{equation}
    R_{\text{force, thumb}} = I(0.01 \le F_{\text{thumb}} \le 200),
\end{equation}

\begin{equation}
R_{\text{force}, i} = \exp\left(-\frac{(F_i - F_{\text{target}})^2}{2\sigma^2}\right) \cdot I(0.01 \le F_i \le 200) ,\quad
\end{equation}
where $F_i$ is the fingertip contact force of the root joint (finger $i$), $\sigma$ is the standard deviation of the Gaussian function, set at 0.10, $I(\cdot)$ is the indicator function.

In addition to standard grasping rewards, we introduce a novel four-finger consistency reward to promote coordinated motion among the four homologous and structurally similar fingers. This term regulates the uniformity of their flexion and extension angles. In the human hand, biomechanical constraints limit the range of independent motion of the metacarpophalangeal joints, causing adjacent fingers to move correlatively. In contrast, robotic fingers are driven by independent motors. Without explicit coordination, reinforcement learning policies often produce unnatural and inefficient postures. The consistency reward encourages more human-like motion patterns, leading to more stable and physically plausible grasps with improved force distribution.

The four-finger difference penalty $R_{\text{diff}}$ is defined as:
\begin{equation}
  R_{\text{diff}} = w_{\text{diff}} \cdot \text{Var}(\{q_j \mid j \in \text{inner fingers}\})  ,
\end{equation}
where $w_{\text{diff}}$ is the penalty weight, $q_j$ is position of the first joint of finger j, $\text{Var}(\cdot)$ is variance of the set of joint positions.

The outer finger movement penalty $R_{\text{outter}}$ is defined as:
\begin{equation}
    R_{\text{outter}} = w_{\text{outter}} \cdot \|{q_{\text{outter}}} - {c_{\text{outter}}}\|_2,
\end{equation}
where $w_{\text{outter}}$ is the weight of this penalty, ${q_{\text{outter}}}$ is current joint position vector for the outer joints (index, middle, ring, and little fingers), ${c_{\text{outter}}}$ is center position vector of the outer joints.

Also, several standard penalty terms are incorporated to refine the agent's behavior. A terminal state penalty is applied to prevent premature termination of the task. Furthermore, we penalize significant changes in action commands between consecutive time steps to encourage smoother control policies. This is formulated as the action rate penalty:
\begin{equation}
R_{\text{action}} = w_{\text{action}} \cdot \|{a}_t - {a}_{t-1}\|_2^2,
\end{equation}
where $R_{\text{action}}$ is the action rate penalty, $w_{\text{action}}$ is the weight of this penalty, ${a}_t$ is the action vector at the current time step $t$, and ${a}_{t-1}$ is the action vector at the previous time step $t-1$.
And a joint velocity L2 penalty to discourage high joint velocities. This encourages the agent to generate smoother and more stable movements, avoiding abrupt motions. The penalty is defined as:
\begin{equation}
R_{\text{vel}} = w_{\text{vel}} \cdot \|\dot{{q}}\|_2^2,
\end{equation}
where $\dot{{q}}$ represents the joint velocity vector, and $w_{\text{vel}}$ is the corresponding penalty weight.

\subsubsection{In-Hand Object Rotation}


\begin{table}[]

\centering
\begin{tabular}{@{}c|c|c@{}}
\toprule
Reward & Formula & Weight \\ \midrule
Close to goal & $ \frac{1.0}{|d_{rot}| + \epsilon}\times \frac{1}{1 + e^{400 (d_{goal} - 0.05)}}$ & 1.0 \\
Action penalty & $||{{a}_t - {a}_{t-1}}||^2$ & -0.0002 \\ \midrule
Reset reward & Condition & Value \\ \midrule
Reach goal bonus & $d_{rot}<0.3$ and $d_{pos}<0.05$ & 250 \\ \bottomrule
\end{tabular}
\caption{Reward for in-hand object rotation}

\label{tab:cube_reward}
\end{table}

To mitigate the sim-to-real gap for rotating objects, we utilize observations that are commonly available in the real world, as shown in Tab.~\ref{tab:obs_rotate}. We implemented and successfully trained two types of policies: one without the direct measurement of object orientation, and the other with the feedback of the object orientation measured via an embedded IMU directly. 

The first type of policy excludes the relative target orientation from the observations and relies solely on the proprioceptive information of the dexterous hand to rotate the object. The second type of policy uses a low-cost IMU sensor embedded inside the object to obtain its orientation directly, and computes the relative rotation to the target. In particular, the technical know-how is to represent the orientation in a 6D continuous format~\cite{zhou2019continuity}, because we found that the quaternion representation has a fundamental double-cover problem: every 3D rotation can be represented by two unit quaternions, q and -q, which correspond to the exact same orientation. This mathematical property creates an undesired discontinuity in the parameter space, disrupting policy learning. In contrast, the 6D rotation representation provides a continuous and smooth mapping, which in turn makes the loss function continuous and relatively smooth in the 6D parameter space.
To encourage continuous rotation, the agent is rewarded for returning the object to a reference position after rotation. However, unconstrained position error $R_{dist}$ initially dominates and creates a local optimum where the agent avoids rotation to preserve reward. To mitigate this, we combine position and rotation error into a single composite reward (Tab.~\ref{tab:cube_reward}), preventing such suboptimal behavior and promoting continuous in-hand manipulation.

\subsection{Sim-to-Real Transfer}


We identified three primary contributors to the sim-to-real gap in our task: tactile sensing, complex in-hand contact simulation, and actuator dynamics. Our approach closes this gap through precise problem formulation and tailored simulation techniques.

\subsubsection{Tactile Sensor Simulation}

We implement a rapid, massively tactile sensor simulation using parallel forward kinematics, which calculates the distance from each sensor unit to the N-nearest surface points on the object.


We consider a dexterous hand with \(N\) fingers. Typically, \(N = 5\). The sensor set of the entire dexterous hand can be denoted as \(S\). On the fingertip of each finger \(i\) (where \(i \in \{1, 2, \ldots, N\}\)), there is a set of sensors, which we represent as \(S_i\). Therefore, the total sensor set is the union of all fingertip sensor sets:
\[ S = \bigcup_{i = 1}^{N} S_i. \]
For each individual sensor \(j\) on each fingertip \(i\) (where \(j \in \{1, 2, \ldots, M_i\}\), and \(M_i\) is the total number of sensors on the \(i\) - th fingertip), we define its key attributes:


\textbf{Position}: Through forward kinematics, we can calculate the spatial coordinates of each sensor from the hand degrees-of-freedom position, denoted as \(p_{ij} \in \mathbb{R}^3\).


\textbf{Activation}: On the real robot hand, the sensor is activated while reading is greater than a threshold. In the simulation, as shown in Fig.~\ref{fig:contact}, the nearest point ${p}_o$ on the surface of the object is found for each sensor ${p}_{ij}$. A vector from the object pointing to each \textit{tacxiel}, ${v}_{oij}$, is defined. The contact is detected if the sensor has deformed, which is determined by evaluating the dot product of ${v}_{oij}$ and the normal vector of the object at ${p}_o$. The vector from ${p}_o$ to ${p}_ij$ is given by:${v}_{oij} = {p}_{ij} - {p}_o$. Let ${n}_o$ be the outward-pointing normal vector at the object point ${p}_o$. If the dot product of ${v}_{oij}$ and ${n}_o$ is negative, it implies that the sensor has penetrated the object's surface, indicating a deformation. All points meeting such a condition are considered as \textit{equivalent contact points}.
    \begin{equation}
         \text{Contact} \iff {v}_{oij} \cdot {n}_o < 0 .
    \end{equation}

    
\textbf{Force}: On the real robot, normal forces are measured by the sensors. In the simulation, it is approximated using Mooney-Rivlin stress: strain relationship model to quantify the contact force of each sensor based on the distance $d_{ij} =|v_oij|$ between the sensor and the object surface and the total contact force per finger, denoted as \(f_{ij} \in \mathbb{R}^+\). 
% On the real robot, contact force is measured directly. In simulation, it is approximated using a Mooney-Rivlin material model, where the force on each sensor is derived from its distance dijdij​ to the object surface and the total contact force per finger.

In our model, we use the fully actuated robotic hand Xhand with 12 degrees of freedom. Each fingertip has \(M_i = 120\) sensors, so the entire hand has \(\sum_{i = 1}^{N}M_i = 600\) sensors. These sensors are concentrated in five independent ``dense groups''. This high local resolution on each fingertip can capture fine pressure distributions.

\subsubsection{Complex Contact Simulation}

The simulation of intricate in-hand contacts is made more robust by randomizing the coefficients for surface friction, damping, and restitution.


\textbf{Modeling of Tactile Sensors:} Building on the dual characteristics of contact sparsity and high resolution, the tactile information from each fingertip is denoted as $T_i$ to represent and process the tactile data. This modeling approach preserves critical contact states while accommodating the spatial sparsity of the data. $T_i$ is defined as:
\begin{equation}
    T_i = (F_i, {\mu}_i).
\end{equation}
where $F_i$ is the total contact force, ${\mu}_i$ is the Force-weighted Mean Contact Position.


\textbf{Total Contact Force ($F_i$):}
The resultant contact force $F_i$ is defined on the real robot as the sum of the total forces from all active sensors on the $i$-th fingertip. In simulation, it is the resultant force between the fingertip and the object, reflecting the effect of all the finger-object point-contacts:
\begin{equation}
    F_i = \sum_{j \in S_i^*} f_{ij}.
\end{equation}



\textbf{Force-weighted Mean Contact Position (${\mu}_i$):}
The mean contact position ${\mu}_i \in \mathbb{R}^3$ is a force-weighted average position that represents the center of pressure:
\begin{equation}
    {\mu}_i = \frac{\sum_{j \in S_i^*} f_{ij} \cdot {p}_{ij}}{F_i}.
\end{equation}
Here, the position of each active sensor, ${p}_{ij}$, is weighted by its force value, $f_{ij}$. The denominator, $F_i$ (the total contact force), ensures this is a normalized weighted average. In a simulation environment, this process can be simplified to:


\begin{align}
      {\mu}_{i,sim} &=  \frac{\sum_{j \in S_i^*} d_{ij}\cdot k \cdot {p}_{ij}}{D_i\cdot k}\nonumber =\frac{\sum_{j \in S_i^*} d_{ij}\cdot {p}_{ij}}{D_i} .
\end{align}

As illustrated in Fig.~\ref{fig:contact_point}, we plot force-weighted contact centers and force magnitudes during an object selection task performed by a dexterous hand in both real-world and simulation environments. It can be observed that the distributions of force-weighted contact centers and force magnitudes exhibit high similarity between the real world and simulation. Furthermore, the real-world contact region is contained within the simulation contact region, demonstrating that contact features can be effectively transferred from simulation to the real world.
\subsubsection{Current-torque Calibration}
To calibrate real-world motor current and simulated joint torque with contact force, we applied varying forces to each fingertip in both real and simulated environments. Real-world motor current and tactile sensor readings were recorded, while joint torque and applied force magnitudes were collected in simulation. Scatter plots and fitted curves (Fig.~\ref{fig:fig_force}) show a proportional relationship between contact force and both current and torque. We recorded the maximum current $I_{max}$, maximum torque $\tau_{max}$, and their corresponding maximum contact forces $F_{max,real}$ and $F_{max,sim}$.  These values were normalized to $[0, 1]$, aligning real-world current with simulated torque and their respective contact forces.


\subsubsection{Actuator Model Randomization}

%To bridge the sim-to-real gap in dexterous manipulation, we propose a randomized actuator model that captures the non-ideal characteristics of physical motors, including torque-velocity saturation and backlash hysteresis. This randomization improves policy robustness against the variations and non-linearities encountered on real hardware. The control torque is computed using a PD controller with randomized gains:

To bridge the sim-to-real gap in dexterous manipulation, we use a randomized actuator model that captures real-world motor nonlinearities—such as torque-velocity saturation and backlash hysteresis—improving policy robustness against hardware variations. The torque is computed via a PD controller with randomized gains:
\begin{equation}
\tau_c = k_p \cdot \left( q_{\text{ref}} - q_m \right) + k_d \cdot \left( \dot{q}_{\text{ref}} - \dot{q}_m \right),
\end{equation}
where $k_p$ and $k_d$ are the proportional and derivative gains, respectively, and $q_m$ denotes the measured joint position.

A key feature of the model is the incorporation of backlash, simulating mechanical dead zones due to gear play. The effective torque is modulated by a deadband function:
\begin{equation}
\tau_b = 
\begin{cases} 
0 & \text{if } |q_{\text{ref}} - q_m| < \epsilon \\
\tau_c & \text{otherwise}
\end{cases},
\end{equation}
where $\epsilon$ is the backlash threshold, randomized during training to mimic physical wear and tolerance variations.

Further, the torque is constrained by a velocity-dependent saturation function due to the DC motor's characteristics:
\begin{align}
\tau_{\text{sat}}^{+}(\dot{q}) = \tau_0 \left(1 - \frac{|\dot{q}|}{\dot{q}_{\text{max}}}\right), \hspace{2mm}
\tau_{\text{sat}}^{-}(\dot{q}) = -\tau_0 \left(1 - \frac{|\dot{q}|}{\dot{q}_{\text{max}}}\right),
\end{align}
where $\tau_0$ is the stall torque and $\dot{q}_{\text{max}}$ is the maximum no-load velocity. The final applied torque is given by:
\begin{equation}
\tau_{\text{applied}} = \eta \cdot \text{clip}\left( \tau_b,\ \tau_{\text{sat}}^{-}(\dot{q}),\ \tau_{\text{sat}}^{+}(\dot{q}) \right),
\end{equation}
where $\eta$ is a randomized factor that accounts for variations in motor torque constant and drive efficiency.

All model parameters are resampled for each actuator at the beginning of every training episode. This comprehensive randomization strategy forces the control policy to adapt to a wide spectrum of actuator imperfections, significantly improving sim-to-real transfer performance.



\section{Experimental Results}
\label{sec:exp}





\subsection{Force-adaptive grasping}We conducted an ablation study on the reward terms 
$R_{\text{Force}}$ and $R_{\text{torque}}$, which are designed to regulate grasping force magnitude. As summarized in Tab.~\ref{tab:abl_force}, using both terms together leads to stronger and wider ranges of contact forces and joint torques, reflecting more forceful and dynamic grasping.
When only $R_{\text{Force}}$ or $R_{\text{torque}}$ is used, both the contact force and joint torque ranges are reduced, indicating less assertive grasping. These findings confirm that both reward components are necessary for achieving robust and adaptive grasping.


Further, we investigated the relation of contact force and torque as functions of the force command, as shown in Fig.~\ref{fig:Force_command}. Both contact force and torque exhibit an approximately linear positive correlation with the commanded force intensity. It can be observed that the strength of correlation decreases in the following order: when both reward terms are used, when only 
$R_{\text{Force}}$ is used, and when only $R_{\text{torque}}$ is applied.

\subsection{In-Hand Object Rotation}

We conducted real-world ablation experiments to assess each observation component. Policies were evaluated on ten trials using consecutive successes, average duration, and time to failure as metrics (Tab.~\ref{tab:abl_cube}). The full configuration—force-weighted contact center, contact force, and 6D orientation—achieved optimal performance with 25.1 consecutive successes and a 3.36-second average duration. Replacement of 6D with quaternions caused a significant decrease to 2.9 successes, showing the need for a continuous rotation representation. Removing the force-weighted contact center reduced successes to 12.2, while omitting contact force resulted in 13.2 successes. Ablating both components further decreased performance to 7.5 successes. The baseline without contact sensing performed poorly (1.1 successes), confirming the need for tactile feedback. A model without explicit orientation encoding had 11.2 successes, underperforming the full configuration. These results show that contact information, force sensing, force weighting, and 6D rotation are critical to robust in-hand rotation.

\subsubsection{Visualization Results} As shown in Fig.~\ref{fig:grasp} and Fig.~\ref{fig:rot_vis}, we present simulation and real-world results for both force-adaptive grasping and in-hand rotation. The policies exhibit consistent behavior across domains. Fig.~\ref{fig:grasp_force_command} further demonstrates the response to different force commands, showing that the policy modulates grasp intensity as intended. Moreover, Fig.~\ref{fig:irregularly} illustrates successful grasping of unseen irregular objects, indicating that the policy generalizes to novel shapes with stable and conforming contact.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]

\centering
\begin{tabular}{@{}cc|cc@{}}
\toprule
$R_{\text{Force}}$      & $R_{\text{torque}}$     & Contact force range & Joint torque percent  \\ \midrule
\checkmark & \checkmark &  \numrange[range-phrase ={\,$\sim$\,}]{44.50}{93.92}                   &         \numrange[range-phrase ={\,$\sim$\,}]{1.09}{1.52}               \\
\checkmark & ×           & \numrange[range-phrase ={\,$\sim$\,}]{37.29}{70.02}                     &        \numrange[range-phrase ={\,$\sim$\,}]{0.69}{0.75}                    \\
          × & \checkmark &      \numrange[range-phrase ={\,$\sim$\,}]{38.45}{47.12}               &            \numrange[range-phrase ={\,$\sim$\,}]{0.85}{1.02}               \\ \bottomrule
\end{tabular}


\caption{Ablation on the rewards $R_{\text{Force}}$ and $R_{\text{torque}}$. }
\label{tab:abl_force}

\end{table}

\section{Conclusion}
% In this paper, we present an integrated sim-to-real reinforcement learning framework and a whole set of sim-to-real techniques designed to enable robust and force-sensitive hand manipulation on a five-finger dexterous hand. By introducing a fast, approximated modeling of tactile sensors in simulation based on parallel distance computation, we enabled high-resolution contact sensing without sacrificing training speed, meanwhile guaranteeing the realism of contact modeling that enables direct sim-to-real transfer on the real robot. To the best of our knowledge and experience, the simulation techniques presented in this work cover most of the practical needs for the majority of commercially available dexterous humanoid hands on the market, which facilitate the research progress on the learning-based approach for reaching the dexterity of humanoid manipulation capabilities. 

We propose a reinforcement learning framework and a suite of sim-to-real techniques designed to achieve robust, force-aware dexterous manipulation using a five-finger dexterous hand. To overcome the challenge of simulating tactile sensing without incurring high computational costs, we introduce a novel approximation method based on parallel distance computation. This approach achieves good contact approximation that enables zero-shot sim-to-real transfer, while ensuring the high sample efficiency required for training in simulation. To the best of our knowledge and experience, our simulation-based RL techniques are broadly applicable for training dexterous manipulation policies on a wide range of commercial humanoid hands, thereby facilitating research progress toward human-level dexterity via simulation-based learning paradigm.



==> sections/conclusion.tex <==
\section{Conclusion}

==> sections/contribution.tex <==
\section{Contributions \& Acknowledgements}

==> sections/data_training.tex <==
\section{Training Recipe}
\label{sec:data_training}

==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

==> sections/introduction.tex <==
\section{Introduction}
\label{sect:intro}
Multi-finger dexterous hands offer human-like manipulation potential, yet their high degrees of freedom (DoFs) and complex contact dynamics pose substantial control challenges. As a result, most robotic applications still rely on simpler parallel-jaw grippers, and achieving robust in-hand manipulation remains a research challenge in robotics.

%This research particularly investigates the use of \emph{full-state} feedback, including tactile sensing and joint torques, for learning manipulation policies that can explicitly sense and regulate contact. In contrast to vision- or kinematics-only approaches, we feed the policy with high-resolution tactile feedback \emph{and} joint-level torques, which represent the interaction forces exerted by multi-fingers. With use of “touch-and-torque” observation, we formulate the reinforcement learning (RL) objectives to achieve effective learning of two essential manual skills—(i) \emph{controllable grasping} (tracking commanded grip forces), and (ii) \emph{in-hand reorientation}.

This work focuses on using the \emph{full-state} feedback, including tactile sensing and joint torques, to learn manipulation policies capable of explicitly sensing and regulating contact. Unlike vision- or kinematics-only methods, our policy uses high-resolution tactile sensing and joint-level torques, capturing fine-grained interaction forces during multi-finger manipulation. This ``touch \& torque'' observation supports reinforcement learning (RL) objectives for two fundamental manual skills: (i) force-controllable grasping (tracking commanded grip forces), and (ii) in-hand reorientation.

Deep reinforcement learning (RL) has begun to unlock dexterous in-hand skills. A landmark result trained a five-finger hand to rotate objects purely in simulation and transferred it to a real robot via large-scale domain randomization~\cite{andrychowicz2018learning}, with subsequent work culminating in automatic domain randomization for a Rubik’s Cube~\cite{akkaya2019rubik} and establishing sim-to-real as a key tool~\cite{tobin2017dr}. 

%Deep reinforcement learning (RL) has emerged as a promising approach for dexterous in-hand manipulation. Related work demonstrated that policies trained in simulation with large-scale domain randomization could be transferred to a real five-finger hand to rotate objects~\cite{andrychowicz2018learning}. Subsequently, automatic domain randomization for a Rubik’s Cube~\cite{akkaya2019rubik} has shown that sim-to-real can be a key tool~\cite{tobin2017dr}. Recent efforts improved simulation fidelity and robustness to train with extensive randomization which yields robust cube reorientation on an Allegro Hand~\cite{handa2023dextreme}. Beyond vision-only policies, recent results integrating tactile sensing has significantly enhanced dexterity, e.g., combining visuotactile and point-cloud inputs~\cite{yuan2023robotsynesthesia} and achieving in-hand rotation using only dense binary touch signals~\cite{yin2023rotating}. Progress also extends to dexterous grasping~\cite{zhang2025robustdexgrasp} and contact-rich humanoid skills~\cite{lin2025humanoid}. Together, these results suggest that with the right sensing and modeling, \emph{sim-to-real RL} can learn manipulation policies readily deployable on real hardware.


Deep reinforcement learning (DRL) has emerged as a promising approach for dexterous in-hand manipulation. Work by ~\cite{andrychowicz2018learning} demonstrated that large-scale domain randomization could transfer simulated object rotation policies to a real five-finger hand. Subsequent advances, such as automatic domain randomization for solving a Rubik’s Cube~\cite{akkaya2019rubik}, and showed sim-to-real as a key tool~\cite{tobin2017dr}. Recent efforts improved simulation fidelity and robustness to train with extensive randomization which yields robust cube reorientation on an Allegro Hand~\cite{handa2023dextreme}. Beyond vision-only policies, integrating tactile sensing has significantly improved dexterity, e.g., fusing visuotactile and point-cloud inputs~\cite{yuan2023robotsynesthesia}, and and achieving in-hand rotation using only dense binary touch signals~\cite{yin2023rotating}. Progress also extends to dexterous grasping~\cite{zhang2025robustdexgrasp}, dexterous in-hand manipulation of thin objects with binary tactile sensing~\cite{hu2025dexterous}, and contact-rich humanoid skills~\cite{lin2025humanoid}. All these results suggest that with the right sensing and modeling, \emph{sim-to-real RL} can learn policies readily deployable on real hardware.


% Recent works report encouraging progress by improving simulation fidelity and policy robustness. ~\cite{handa2023dextreme} demonstrates robust cube reorientation on an Allegro Hand via simulation and extensive randomization. Beyond vision-only policies, integrating tactile sensing can further enhance sim-to-real dexterity: ~\cite{yuan2023robotsynesthesia} fuses visuotactile inputs with a point-cloud tactile representation to perform in-hand rotations, while ~\cite{yin2023rotating} achieves in-hand rotation using only dense binary touch sensing and direct zero-shot deployment. Progress also extends to dexterous grasping: ~\cite{zhang2025robustdexgrasp} reports strong zero-shot grasp success on 500+ real objects, and recent work on humanoids advances sim-to-real RL for contact-rich, vision-based dexterity~\cite{lin2025humanoid}. Together, these results suggest that with the right techniques—better sensing, realistic actuation models, and targeted randomization—\emph{sim-to-real RL} can unlock agile manipulation on real hardware.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{fig/fist_fig.pdf}
    \caption{Learning full-state policy (including tactile sensing and joint torques) for dexterous grasping and in-hand manipulation.}
    \label{fig:placeholder}
    \vspace{-7mm}
\end{figure}

However, there are two practical hurdles for full-state policies that use tactile sensing and joint torques: (i) \textbf{Simulation of dense tactile contacts}. Simulating high-resolution tactile/contact is computationally too slow for massive RL exploration, resulting in a brittle policy due to insufficient exploration of contact dynamics. (ii) \textbf{Discrepancies of actuator dynamics and modeling}. Most dexterous hands have semi-direct-drive actuation with no direct joint torque sensors and thus rely on the motor current to estimate the joint torques, where inaccuracies and uncertainties in the actuator dynamics can hurdle the sim-to-real transfer. In short, major gaps in the \emph{modeling and simulation of surface contacts of tactile sensors and the mechatronic properties of actuators} prevent full-state policies from being fully exploited for policy learning.

% As high-DoF dexterous robotic hands become more commercially available, we are motivated to investigate the sim-to-real \textit{recipe} for learning \textit{full-state policies} for dexterous hands (including tactile sensing and joint torque), to address these bottlenecks by effective modeling of contacts and actuation. Our method trains a policy on a five-finger hand entirely in simulation and deploys it directly to the real world. Specifically, the contribution of sim-to-real \textit{recipe} includes:

As high-DoF dexterous hands become more available, we are motivated to develop a reliable sim-to-real \textit{recipe} for learning full-state policies (including tactile sensing and joint torques) that address key sim-to-real gaps through effective modeling of tactile sensors and actuators. Our method trains a policy in simulation and deploys it directly to a real five-finger hand. The contributions of this \textit{recipe} include:
\begin{itemize}
[leftmargin=*]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
\item \textbf{Full-state policies.} We formulate the policy observations that jointly intake dense tactile sensing and joint torques, enabling explicit feedback that can infer contact states and contact forces.
\item \textbf{Fast, high-resolution tactile simulation.} We approximate tactile contacts by computing distances between a dense array of \emph{virtual tactile units} and the object via parallel forward kinematics, offering more accurate, high-rate tactile feedback suitable for massive RL training.
\item \textbf{Data-driven actuator modeling.} We bridge the sim-to-real actuation gap by calibrated current-to-torque mapping and randomization to account for uncertain motor dynamics (e.g., torque-velocity curves), requiring no direct torque sensors and reducing sim-to-real torque discrepancies on real hardware.
% \item \textbf{Motor dynamics modeling and randomization.} We capture non-idealities (e.g., torque–speed limits) and randomize key parameters during training to bridge actuation gaps.
\item \textbf{Contact-rich sim-to-real RL policy training.} We trained and deployed two contact-rich skills: (1) \emph{controllable grasping} that tracks commanded grip forces and (2) \emph{in-hand object reorientation} -- full-state policies directly deployed for force-modulated grasps and reorientations on the real robot.
\end{itemize}

%In summary, we contributed an easy-to-replicate \textit{recipe} for training full-state RL policies on a representative dexterous hand (12-DoF) widely available for robotics research. By combining tactile/torque-aware observations with approximate tactile simulation, actuator calibration, and modeling of motor dynamics, our \textit{recipe} achieves zero-shot transfer of \emph{force-controllable} grasping and in-hand reorientation with policies trained entirely in simulation. To the best of our knowledge, this is the first demonstration of \emph{controllable grasping} with controllable grip-force tracking, force-adaptive grasping, and robust in-hand manipulation on a dexterous multi-finger hand.

In summary, this serves as an easy-to-replicate \textit{handbook} for training full-state RL policies on a representative dexterous hand (12-DoF) widely available recently for robotics research. Our approach integrates tactile and motor-current sensing with computationally efficient simulation and robust actuator modeling, enabling zero-shot sim-to-real transfer of force-controllable grasping and in-hand manipulation. To the best of our knowledge, this is the first demonstration of \emph{controllable grasping} with grip-force tracking, force-adaptive grasping, and robust in-hand manipulation on a dexterous multi-finger hand.

%To the best of our knowledge, this is the first demonstration of direct sim-to-real transfer of force-sensitive dexterous manipulation on a multi-fingered hand.


==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sect:preliminaries}


==> sections/relatedwork.tex <==
\section{Related Work}
